Latent Bridges for Multi-Table Question Answering

We introduce GRAB, a constructor-encoder-bridge pipeline for table question answering. Our method lifts relational data into an heterogeneous graph, encodes it via message passing, and transfers the signals to an LLM through a small set of query-conditioned latent tokens. This provides the LLM with a compact, task-relevant structural representation together with the flattened text. Crucially, the LLM remains strictly frozen to preserve its general reasoning capabilities; we train only the lightweight graph encoder and latent bridge (91M parameters), allowing the entire pipeline to be trained efficiently. Our pipeline significantly improves performance on relational Question Answering, with the largest gains in demanding multi-table settings, offering an efficient, principled way to connect relational deep learning with LLMs.

==> sec4-old.tex <==
As illustrated in Figure \ref{fig:architecture}, 
instead of relying only on $S_{\text{\sl table}}$, we define a \textit{graph constructor} $\gamma$ that lifts the relational context into an explicit heterogeneous graph $\cG=\gamma(\cT,\cF)$, where rows, column classes, and value groups are represented as typed nodes and foreign-key metadata induces shared column classes. A graph encoder processes $\cG$ to capture row--column--value dependencies and cross-table connectivity. To interface with the LLM, we define a query-conditioned latent bridge that projects the encoded graph into a fixed-length sequence of $K$ soft tokens, denoted $Z=\{z_1,\dots,z_K\}$. The LLM then generates the answer from both the textual prompt and %the graph-derived 
our structural prefix. Throughout this process, the LLM weights remain frozen. %; only encoder and bridge are updated.


% Following the formalization of \citet{grables}, instead of relying on $S_{table}$, we define a \textit{graph constructor} $\gamma$ that lifts the relational context into an explicit heterogeneous graph $\mathcal{G} = \gamma(\mathcal{T}, \mathcal{M})$, where rows and values are mapped to canonical nodes, and relationships in $\mathcal{M}$ define structural edges. A graph encoder processes $\mathcal{G}$ to capture these cross-table dependencies. To interface with the LLM, we define a {query-conditioned} latent bridge that projects the encoded graph into a fixed-length sequence of $K$ soft tokens, denoted $Z = \{z_1, \dots, z_K\}$. Consequently, the LLM generates the answer by modeling $P(A \mid Q, Z)$, effectively replacing brittle text serialization with a query-conditioned structural summary.

% Consequently, the LLM generates the answer together with a query-conditioned structural summary. Throughout this process, the LLM weights remain entirely frozen; only the 63M parameters of the graph encoder and latent bridge are updated, ensuring high training efficiency and zero disruption to the LLM's foundational behavior.

\stitle{Relational Graph Constructor.}
%\label{sec:constructor}
The \textit{graph constructor} $\gamma$ is a fixed, deterministic processing map. It  exposes row--column--value incidence and cross-table join structure before any neural message passing occurs. Let $\cF$ denote the foreign-key metadata in $\mathcal{M}$:
$\cF =
\bigl\{\bigl((i,c),(j,d)\bigr) \mid
\text{column  $c$  of $T_i$ joins
column $d$ of  $T_j$}\bigr\}.$
%We assume that column types agree for every foreign-key link.

The constructor maps the relational input to a tripartite graph
$\gamma(\cT,\cF) =
\bigl(\cG,\bH^{(0)}\bigr)$, with $
\cG =
\bigl(
\cV_R\cup\cV_C\cup\cV_V,
\cE_{RV}\cup\cE_{CV}
\bigr)$,
where $\cV_R$ are row nodes, $\cV_C$ are column-class nodes, $\cV_V$ are value-group nodes, $\cE_{RV}$ are row--value incidence edges, and $\cE_{CV}$ are column--value incidence edges. Furthermore,
$\bH^{(0)}=\{\bh^{(0)}_v\}_{v\in\cV_R\cup\cV_C\cup\cV_V}$ are the initial node features.  In more detail:

\textit{Column classes.}
Let
$\cC_{\mathrm{occ}}
=
\{(i,c) \mid i\in[n],\, c\in C_i\}$
be the set of column occurrences across all tables. The relation $\sim_{\cF}$ is the smallest equivalence relation on $\cC_{\mathrm{occ}}$ containing all foreign-key pairs in $\cF$. We write $[(i,c)]_{\cF}$ for the equivalence class of column occurrence $(i,c)$, and use $\alpha$ for a generic class. When $\cF=\emptyset$, the relation is the identity and no columns are merged. We denote the set of column classes by
$\cC_{\cF} = \cC_{\mathrm{occ}}/\!\sim_{\cF}$. For example, in Figure~\ref{fig:architecture}, the city columns in $T_1$ and $T_2$ map to a single node in $\mathcal G$.
Each class $\alpha$ inherits a single type $\tau_\alpha\in\{\mathrm{cat},\mathrm{num},\mathrm{text}\}$. 

\textit{Nodes.}
Row nodes are indexed globally across tables, column nodes correspond to FK-induced column classes, and value nodes correspond to canonical value groups within a column class:
$
\cV_R
=
\bigl\{\rho_{i,r} \mid i\in[n],\, r\in R_i\bigr\}$,
$\cV_C
=
\bigl\{c_\alpha \mid \alpha \in \cC_{\cF}\bigr\}$, and
$\cV_V
=
\bigl\{v_{\alpha,g}
\mid
\alpha \in \cC_{\cF},\,
g\in\mathrm{Im}(g_\alpha)
\bigr\}
$.
Here, for each column class $\alpha$, the grouping map $g_\alpha$ standardizes cell contents:
\[
g_\alpha(x)
=
\begin{cases}
\mathrm{id}_\alpha\bigl(\mathrm{norm}(x)\bigr),
& \tau_\alpha\in\{\mathrm{cat},\mathrm{text}\},\\[2pt]
q_\alpha(x),
& \tau_\alpha=\mathrm{num}.
\end{cases}
\]
%For categorical and textual columns, 
where $\mathrm{norm}(\cdot)$ normalizes the cell string and $\mathrm{id}_\alpha(\cdot)$ assigns a unique identifier to each distinct normalized value within $\alpha$, while %. For numeric columns, 
$q_\alpha(\cdot)$ maps values to quantile-based buckets fitted on all numeric values in the class. A value node $v_{\alpha,g}$ therefore represents a repeated categorical/textual value or a numeric range, not an individual cell occurrence.\footnote{Value groups are not replacements for exact numeric content, which remains available in the textual prompt.}

\textit{Edges.} 
For each cell $x^{(i)}_{r,c}$ (value in column $c$ in row $r$ in $R_i$),
let $\alpha=[(i,c)]_{\cF}$ and $g=g_\alpha(x^{(i)}_{r,c})$. The constructor adds the row--value edge
$\{\rho_{i,r},v_{\alpha,g}\}$ to $\cE_{RV}$ and the column--value edge
$\{c_\alpha,v_{\alpha,g}\}$ to $\cE_{CV}$. Thus, repeated values become shared graph neighborhoods, and foreign-key joins become explicit connectivity through shared column classes and value groups. % rather than only textual context.

\textit{Initial features.}
Let $\phi_{\mathrm{tok}}$ be a fixed token-level text encoder. For any string
$s\in\Sigma^*$, define 
$\phi(s)$ as $
\mathrm{MeanPool}\bigl(\phi_{\mathrm{tok}}(s)\bigr)$.

The graph's hidden feature dimension is inherited from the embedding model used to
initialize the nodes. In our implementation, row and column nodes are initialized
from the same text embedding model, while value nodes are constructed directly
in the same hidden dimension. Therefore, all node types already lie in a common  
embedding space and no additional projection is applied at initialization. We
write $\Vert$ for string concatenation.

For a row node $\rho_{i,r}$, we encode a row-level string formed by
concatenating header--value pairs:
\[
s_{i,r}
=
\big\Vert_{c\in C_i}
\bigl[\,h^{(i)}_c : x^{(i)}_{r,c}\,\bigr],
\qquad
\bh^{(0)}_{\rho_{i,r}}
=
\phi(s_{i,r}).
\]

For a column node $c_\alpha$, we initialize from the header embedding of the
corresponding column occurrence. If $\alpha$ contains multiple
FK-linked column occurrences, we average their header embeddings
$
\bh^{(0)}_{c_\alpha}
=
\frac{1}{|\alpha|}
\sum_{(i,c)\in\alpha}
\phi\bigl(h^{(i)}_c\bigr)$.

For a value node $v_{\alpha,g}$, we do not initialize from the cell-value text.
Instead, we use a deterministic embedding of the value-group identifier,
augmented with the column-type information, constructed in the graph
hidden dimension. Thus, value nodes primarily act as structural anchors: they
indicate where identical categorical/textual values or discretized numeric
buckets occur, while exact values are available to the LLM with
$S_{\text{\sl table}}$.

% Let $\phi_{\mathrm{tok}}$ be a fixed token-level text encoder. For any string $s\in\Sigma^*$, define
% $\phi(s)
% =
% \mathrm{MeanPool}\bigl(\phi_{\mathrm{tok}}(s)\bigr)$.

% \redtext{Simone: the graph dimension is based on the embedding model used to initialize the row/col nodes so there is no projection since they are initialized with the same model}

% Let $\bW_R,\bW_C,\bW_V$ be projection matrices to the graph hidden dimension $d_h$, and let $\be_\tau$ be a type embedding for each $\tau\in\{\mathrm{cat},\mathrm{num},\mathrm{text}\}$. We write $[\,\cdot\,;\,\cdot\,]$ for vector concatenation and $\Vert$ for string concatenation.

% For a row node $\rho_{i,r}$, we encode a row-level string formed by concatenating header--value pairs:
% \[
% s_{i,r}
%  =
%  \big\Vert_{c\in C_i}
%  \bigl[\,h^{(i)}_c : x^{(i)}_{r,c}\,\bigr],
%  \qquad
%  \bh^{(0)}_{\rho_{i,r}}
%  =
%  \bW_R\,\phi(s_{i,r}).
% \]
% \redtext{Simone: each column header is initialized alone, the avg is done only if there is the merge with fk}
% For a column node $c_\alpha$, we initialize from the mean-pooled encodings of all headers in the class:
% \[
% \bh^{(0)}_{c_\alpha}
%  =
%  \bW_C\!\left(
%  \frac{1}{|\alpha|}
%  \sum_{(i,c)\in\alpha}
%  \phi\bigl(h^{(i)}_c\bigr)
%  \right).
% \]
% For a value node $v_{\alpha,g}$, we do \emph{not} initialize from the cell-value text. Instead, let $\bu_{\alpha,g}\in\bbR^{d_g}$ be a deterministic embedding of the group identifier $g$ within class $\alpha$. We set
% \[
% \bh^{(0)}_{v_{\alpha,g}}
%  =
%  \bW_V\bigl[\,\bu_{\alpha,g};\,\be_{\tau_\alpha}\,\bigr].
% \]
% Value nodes therefore act primarily as structural anchors: they indicate where identical categorical/textual values or discretized numeric buckets occur, while exact surface values remain available to the LLM through $S_{\mathrm{table}}$.
% \subsection{Relational Graph Constructor}
% % Hints:
% % - Define how one or multiple tables are converted into a heterogeneous graph.
% % - Specify node types (e.g., table, row, column, value, key, schema node).
% % - Specify edge types (e.g., incidence, same-row, same-column, PK-FK, schema edges).
% % - Clarify whether the constructor is fixed, learned, or partially learned.
% % - Emphasize why joins become first-class structural relations here.
% The \textit{graph constructor} $\gamma$ is a fixed and deterministic processing map. For each sample, it creates a tripartite graph whose nodes correspond to rows, columns and value groups. In single-table scenario, the table is mapped to a graph $\mathcal{G} = (\cV_R \cup \cV_C \cup \cV_V,  \cE_{RV} \cup \cE_{CV})$, where $V_R$ is the row nodes set, $V_C$ the header nodes set and $V_V$ the value/group nodes, while
% $E_{RV}$ contains row-value incidence edges and
% $E_{CV}$ contains column-value incidence edges. In the multi-table case, row and column nodes are indexed globally across all tables, and each row and column node is associated with its
% source table identity. When foreign-key metadata is available, columns participating in the same relational are represented with the same  column node, so join relations become explicit graph connectivity rather than only textual context.
% Value groups are created by standardizing the contents of cells within each column. 
% For categorical or textual cells, the constructor normalizes the cell string and assigns identical values in the same column to the same value-group identifier. For numeric columns, its values are discretized into quantile-based buckets, and each bucket is treated as a value group \footnote{Value groups are not replacements for exact numeric content, which remains available in the textual prompt.}. 
% Thus, a value node may represent either a repeated categorical value or a numeric range rather than an individual cell occurrence. 
% After constructing the graph topology, the constructor assigns an initial feature vector to each node type. 
% Row nodes are initialized by encoding a row-level textual representation, obtained by concatenating the cells in the row with their column names and then mean-pooling the embeddings obtained from the sequence. Column nodes are initialized from the encoded column headers. Value nodes, in contrast, are not initialized from the textual content of the
% cell values. Instead, they are initialized from their value-group identifiers, augmented with column-type embeddings. Thus, value nodes primarily act as structural anchors: they indicate where identical categorical values or discretized numeric buckets occur in the table. These initial states are then passed to the graph encoder for message propagation.


==> tables/tab_GNN-depth.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{ccccccc}
\toprule
\textbf{Layers} & \textbf{StructQA} & \textbf{HiTab} & \textbf{MultiHierTT} & \textbf{MMQA} & \textbf{Avg} \\
\midrule
1  & 0.8313 & 0.7431 & 0.2213 & 0.3014 & 0.5243 \\
2 & 0.8073 & 0.7373 & 0.1887 & 0.3134 & 0.5104 \\
4  & 0.8287 & 0.7367 & 0.2117 & 0.2943 & 0.5179 \\
8  & 0.8320 & 0.7399 & 0.2155 & 0.3014 & 0.5222 \\
\textbf{16} & \textbf{0.8400} & \textbf{0.7544} & 0.2203 & 0.2895 & \textbf{0.5261} \\
\bottomrule
\end{tabular}
\caption{GNN depth ablation. We vary the number of message-passing layers with $K{=}32$ latents and resampler fixed. Bold denotes the best result per column.}
\label{tab:gnn_depth_ablation}
\end{table}

==> tables/table-computational-overhead.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrr}
\toprule
& Serialized & GRAB \\
\midrule
Decoding latency (ms/token) & 21.4 & 23.1 \\
Compute (TFLOPs/query)      & 6.47 & 7.26 \\
Peak GPU memory (GB)        & 7.98 & 8.43 \\
%Trainable parameters        & --   & 91M \\
\midrule
End-to-end inference (s)    & 1101 & 830 \\
Mean generated tokens       & 23.9 & 21.7 \\
\bottomrule
\end{tabular}
\caption{Computational overhead on the full StructQA test set (1{,}495 queries, frozen Qwen3-4B, batch size 1, CUDA-event timing). The last two rows are behavioral effects of training, not architectural costs.}
\label{tab:overhead}
\end{table}
